Semi-Supervised Action Recognition with Temporal Contrastive Learning

Learning to recognize actions from only a handful of labeled videos is a challenging problem due to the scarcity of tediously collected activity labels. We approach this problem by learning a two-pathway temporal contrastive model using unlabeled videos at two different speeds leveraging the fact that changing video speed does not change an action. Specifically, we propose to maximize the similarity between encoded representations of the same video at two different speeds as well as minimize the similarity between different videos played at different speeds. This way we use the rich supervisory information in terms of `time' that is present in otherwise unsupervised pool of videos. With this simple yet effective strategy of manipulating video playback rates, we considerably outperform video extensions of sophisticated state-of-the-art semi-supervised image recognition methods across multiple diverse benchmark datasets and network architectures. Interestingly, our proposed approach benefits from out-of-domain unlabeled videos showing generalization and robustness. We also perform rigorous ablations and analysis to validate our approach. Project page: https://cvir.github.io/TCL/.

==> tables/ablation_selfsupervised.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c}
\hline
Self-Supervised Approach &  Top-1 Accuracy  \\
\hline
0dd-One-Out Networks ~\cite{fernando2017self} & ${19.56}$\\
Memory-augmented Dense Predictive Coding  ~\cite{Han2020Memory} & ${18.67}$\\
Video Clip Order Prediction ~\cite{Xu2019Self} & ${23.93}$\\
\hline
\ours (Ours) & 29.81$\pm{0.77}$\\
\hline
\end{tabular}
} \vspace{-1mm}
\caption{\small \textbf{Comparison with Self Supervised Approaches on Mini-Something-V2.} Numbers show top-1 accuracy with ResNet-18 and 5\% labeled Data. \textcolor{magenta}{Should we rename the first row differenlty as the reviewer 3 had confusion to understand that it is basically a FixMatch with group using temporal info}}
\label{tab:self_supervised} \vspace{-1mm}
\end{table}

==> tables/jester.tex <==
% \begin{table*}[ht]
% \centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\hline
 &  & \multicolumn{3}{c}{Jester} \\  \cline{3-5} Approach &  & 1\% & 5\% & 10\% \\ 
\cline{1-1} \cline{3-5} 
Supervised (8f) & & 52.55 $\pm 4.36$& 85.22$\pm 0.61$& 90.45$\pm 0.48$\\
Pseudo-Label~\cite{Lee2013Pseudo} \small{(\texttt{ICMLW'13})} && 57.99$\pm 3.70$& 87.47$\pm 0.64$& 90.96$\pm 0.48$\\
Mean Teacher~\cite{Tarvainen2017Mean} \small{(\texttt{NeurIPS'17})} &  & 56.68$\pm 1.46$& 88.80$\pm 0.44$& 92.07$\pm 0.03$\\
S4L~\cite{Zhai2019S4L} \small{(\texttt{ICCV'19})}  &  & 64.98 $\pm 2.70$&87.23 $\pm 0.15$& 90.81 $\pm 0.32$\\
MixMatch~\cite{Berthelot2019Mixmatch} \small{(\texttt{NeurIPS'19})} &  & 58.46 $\pm 3.26$& 89.09 $\pm 0.21$& 92.06 $\pm 0.46$\\ 
FixMatch~\cite{Sohn2020Fixmatch} \small{(\texttt{NeurIPS'20})} &  & 61.50 $\pm 0.77$& 90.20 $\pm 0.35$& 92.62$\pm 0.60$\\
\hline 
TCL (Ours)& & 75.21 $\pm 4.48$& 93.29 $\pm 0.24$& 94.64 $\pm 0.20$\\
TCL w/ Finetuning& & 77.25 $\pm 4.02$& 93.53 $\pm 0.15$ & 94.74$\pm 0.25$\\
TCL w/ Pretraining \& Finetuning & & 82.55 $\pm 1.94$& 93.73 $\pm 0.25$& 94.93 $\pm 0.01$\\ 
\hline
\end{tabular}
}
% \caption{Comparison of our proposed approach with image-domain SSL baselines applied to Jester dataset using Resnet-18 backbone model. We report the Top-1 Clip accuracy values in each case.}
% \label{tab:res_jester}
% \end{table*}


==> tables/sthv2.tex <==
% \begin{table*}[ht]
% \centering
% \label{tab:comparison}
% \resizebox{\textwidth}{!}{%
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{tabular}{c||cc|cc|cc||cc|cc|cc}
%  & \multicolumn{6}{c||}{ResNet-18} & \multicolumn{6}{c}{ResNet-50}\\
%  \hline
% \multirow{2}{*}{Approach} & \multicolumn{2}{c|}{1   \%} & \multicolumn{2}{c|}{5   \%} & \multicolumn{2}{c||}{10   \%} & \multicolumn{2}{c|}{1   \%} & \multicolumn{2}{c|}{5   \%} & \multicolumn{2}{c}{10   \%} \\
% \cline{2-13}
% & Clip   acc  & Video   acc  & Clip   acc  & Video   acc  & Clip   acc   & Video   acc  & Clip   acc  & Video   acc  & Clip   acc  & Video   acc  & Clip   acc   & Video   acc  \\
% \hline
% Supervised (8f)                                                                                                          & 6.05        &              & 17.26       & 18.93        & 24.67        &              & 5.69        &              & 16.68       &              & 27.02        &              \\
% PseudoLabel~\cite{Lee2013Pseudo} (\texttt{ICMLW'13}))                              & 6.46        & 6.61         & 18.76       & 19.80        & 25.67        &              & 6.66        &              & 18.77       &              & 28.85        &              \\
% Mean Teacher~\cite{Tarvainen2017Mean} (\texttt{NeurIPS'17})                       & 7.33        &              & 20.23       &              & 30.15        &              & 7.55        &              & 21.80       &              & 32.12        &              \\
% S4L~\cite{Zhai2019S4L} (\texttt{ICCV'19})                                        & 7.18        &              & 18.58       &              & 26.04        &              & 6.87        &              & 17.73       &              & 26.91        &              \\
% MixMatch~\cite{Berthelot2019Mixmatch} (\texttt{NeurIPS'19})                       & 7.45        &              & 18.63       &              & 25.78        &              & 6.48        &              & 17.77       &              & 27.03        &              \\
% FixMatch~\cite{Sohn2020Fixmatch} (\texttt{NeurIPS'20})                           & 6.04        &              & 21.67       & 21.98        & 33.38        &              & 6.54        &              & 25.34       &              & 37.44        &              \\ 
% \hline
% TCL (Ours)                                                                                                            & 7.79        & 8.08         & 29.81       &              & 38.61        &              & 7.54        &              & 27.22       &              & 40.70        &              \\
% \begin{tabular}[c]{@{}c@{}} TCL w/ Fine-tuning \end{tabular}                & 8.65        & 8.88         & 30.55       &              & 40.06        &              & 8.56        &              & 28.84       &              & 41.68        &              \\
% \begin{tabular}[c]{@{}c@{}} TCL w/ Pre-training \& Fine-tuning \end{tabular} & 9.91        & 10.12        & 30.97       &              & 41.55        &              & 9.19        &              & 29.85       &              & 41.90        &             
% \end{tabular}
% }
% \vspace{3mm}
%     \caption{\abir{Give standard deviations. Provide values till 2 decimal places. uns-pretraining is going in two lines. Just use `pretraining'. Do not boldface the values at this moment.} Comparison of our proposed approach with image-domain SSL baselines applied to mini-Something-Something v2 dataset using Resnet-18 and Resnet-50 backbone models. We report the Top-1 accuracy values in each case.}
% \end{table*}

==> tables/supp_cont.tex <==
\begin{table*}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c||c|}
\hline
 Page No. & Contents \\
\hline
\end{tabular}
}
% \caption{Comparison of our proposed approach with image-domain SSL baselines applied to Kinetics dataset using Resnet-18 backbone model. We report the Top-1 Clip accuracy values in each case.}
\label{tab:supp_con}
\end{table*}
